Balancing Statistical and Computational Precision: A General Theory and Applications to Sparse Regression

Modern technologies are generating ever-increasing amounts of data. Making use of these data requires methods that are both statistically sound and computationally efficient. Typically, the statistical and computational aspects are treated separately. In this paper, we propose an approach to entangle these two aspects in the context of regularized estimation. Applying our approach to sparse and group-sparse regression, we show that it can improve on standard pipelines both statistically and computationally.

==> sections/paper2_proofs.tex <==
\section*{Appendix B. Proofs of Section~\ref{sec:paper2}}


\begin{proof}[Proof of Lemma~\ref{lemmageneral}]
Since \subf\, is a subgradient of $f$ at \cm, we find the basic inequality
\begin{equation*}
  1/2\normtwo{Y-X\truth}^2+\tuningparameter\norm{\truth}\geq 1/2\normtwo{Y-X\cm}^2+\tuningparameter\norm{\cm}+\inprod{\subf}{\truth-\cm}.
\end{equation*}
We can now rewrite $\normtwo{Y-X\cm}^2$ as follows:
\begin{align*}
    \normtwo{Y-X\cm}^2 &= \normtwo{Y-X\truth+X\truth-X\cm}^2\\
    &= \normtwo{Y-X\truth}^2 + 2\inprod{Y-X\truth}{X\truth-X\cm}+ \normtwo{X\truth-X\cm}^2\\
    &= \normtwo{Y-X\truth}^2 + 2\inprod{X\tp \left(Y-X\truth\right)}{\truth-\cm}+ \normtwo{X\truth-X\cm}^2.
\end{align*}
Combining the two displays yields
\begin{align*}
\tuningparameter\norm{\truth}\geq \inprod{X\tp \left(Y-X\truth\right)}{\truth-\cm}+ 1/2\normtwo{X\truth-X\cm}^2+\tuningparameter\norm{\cm}+\inprod{\subf}{\truth-\cm}.
\end{align*}
We now use that $\normtwo{X\truth-X\cm}^2\geq 0$ and invoke the model $Y=X\truth+\varepsilon$ to find
\begin{align*}
\tuningparameter\norm{\truth}\geq \inprod{X\tp\varepsilon}{\truth-\cm}+\tuningparameter\norm{\cm}+\inprod{\subf}{\truth-\cm}.
\end{align*}
This can be rearranged to
\begin{align*}
\tuningparameter\norm{\cm}\leq \inprod{X\tp\varepsilon}{\cm-\truth}+\inprod{\subf}{\cm-\truth}+\tuningparameter\norm{\truth}.
\end{align*}
Invoking  H\"older's inequality and the assumptions that $\tuningparameter\geq 2\normd{X\tp\varepsilon}$ and $\normd{\subf}\leq\dif$ provides us with
\begin{align*}
  \inprod{X\tp\varepsilon}{\cm-\truth}+\inprod{\subf}{\cm-\truth}&\leq \normd{X\tp\varepsilon}\norm{\cm-\truth}+\normd{\subf}\norm{\cm-\truth}\\
  &\leq \frac{\tuningparameter}{2}\norm{\cm-\truth}+\dif\norm{\cm-\truth}.
\end{align*}
Together with the above inequality, we thus find
\begin{align*}
\tuningparameter\norm{\cm}&\leq \frac{\tuningparameter}{2}\norm{\cm-\truth}+\dif\norm{\cm-\truth}+\tuningparameter\norm{\truth}\\
&= \left(\frac{\tuningparameter}{2}+\dif\right)\norm{\cm-\truth}+\tuningparameter\norm{\truth}.
\end{align*}
We can decompose each of these vectors into their parts on \superset\ and $\superset^c$. We find
\begin{align*}
 \tuningparameter\norm{\cmsuper}+\tuningparameter\norm{\cmsuperc}&\leq \left(\frac{\tuningparameter}{2}+\dif\right)\norm{\cmsuper-\truthsuper}+\left(\frac{\tuningparameter}{2}+\dif\right)\norm{\cmsuperc-\truthsuperc}+\tuningparameter\norm{\truthsuper}+\tuningparameter\norm{\truthsuperc}\\
 &= \left(\frac{\tuningparameter}{2}+\dif\right)\norm{\cmsuper-\truthsuper}+\left(\frac{\tuningparameter}{2}+\dif\right)\norm{\cmsuperc}+\tuningparameter\norm{\truthsuper}.
\end{align*}
We can rearrange the terms and find
\begin{align*}
    \left(\frac{\tuningparameter}{2}-\dif\right)\norm{\cmsuperc} &\leq \left(\frac{\tuningparameter}{2}+\dif\right)\norm{\cmsuper-\truthsuper}+\tuningparameter\norm{\truthsuper}-\tuningparameter\norm{\cmsuper}.
\end{align*}
Using the reverse triangle inequality, this becomes
\begin{align*}
    \left(\frac{\tuningparameter}{2}-\dif\right)\norm{\cmsuperc} &\leq \left(\frac{3\tuningparameter}{2}+\dif\right)\norm{\cmsuper-\truthsuper}. 
\end{align*}
We can now invoke the assumption $\dif\in [0,\tuningparameter/2)$ to deduce 
\begin{align*}
    \norm{\cmsuperc} &\leq\coneparamnew\norm{\cmsuper-\truthsuper}.
\end{align*}
Finally, setting $\vdiff:=\truth-\cm$ gives the desired inequality
\begin{align*}
    \norm{\vdiffsuperc} &\leq \coneparamnew\norm{\vdiffsuper}. 
\end{align*}
\end{proof}

\begin{proof}[Proof of Theorem~\ref{theoremgeneral}]
A subgradient~\subf\, for the objective function $f$ at \cm\, reads
\begin{equation*}
  \subf = -X\tp(Y-X\cm)+\tuningparameter\vsubc
\end{equation*} 
for a vector \vsubc\ that satisfies $\normd{\vsubc}\leq 1$ and $\vsubc\tp\cm = \norm{\cm}$.
Using the model, we have
\begin{align*}
  \subf=  -X\tp(X\truth+\varepsilon-X\cm)+\tuningparameter\vsubc\,,
\end{align*}
and rearranging yields
\begin{align*}
     X\tp  X(\truth-\cm) &= {\tuningparameter}\vsubc - X\tp\varepsilon - {\subf}\,.
\end{align*}
Applying the dual norm on both sides and using the triangle inequality gives
\begin{align*}
    \normd{X\tp  X(\truth-\cm)} &= \normd{\frac{\tuningparameter}{2}\vsubc - {X\tp\varepsilon} - \frac{\subf}{2}}\\
    &\leq {\tuningparameter}\normd{\vsubc} + \normd{X\tp\varepsilon} +  {\normd{\subf}}\,.
\end{align*}
Using that $\normd{\vsubc}\leq 1$, $\tuningparameter\geq 2\normd{X\tp\varepsilon}$, and $\normd{\subf}\leq \dif$ gives
\begin{align*}
    \normd{X\tp  X(\truth-\cm)} &\leq {\tuningparameter} + \frac{\tuningparameter}{2}+  {\dif}=\frac{3\tuningparameter}{2} + {\dif}\,.
\end{align*}
Now, we recall that  $\vdiff:=\truth-\cm$ satisfies $\norm{\vdiffsuperc}\leq \coneparamnew\norm{\vdiffsuper}$ according to Lemma~\ref{lemmageneral}. Thus, Condition~\ref{conditiongeneral} entails $\normd{\truth-\cm}\leq {\normd{X\tp X(\truth-\cm)}}/{\nobs\supc}$, so that
\begin{align*}
    \normd{\truth-\cm} &\leq \frac{3\tuningparameter}{2n\supc} + \frac{\dif}{2n\supc}
\end{align*}
as desired.
\end{proof}



==> sections/proofs.tex <==
In the first three parts of the Appendix, we introduce the building blocks for proving the claim stated in the main part of the paper, Theorem~\ref{thm:optimality}. Specifically, in Appendix A, we prove a geometric property (Lemma~\ref{cones_cond}) and an oracle inequality (Theorem~\ref{thm:sup_norm_vdiff_main}) for approximate lasso solutions. Next, we show in Appendix B how to verify if the required computational precision is reached (Theorem~\ref{thm:optimality}). Using theses results, we then prove our main result  (Theorem~\ref{thm:optimality})  in Appendix~C. The dependencies among the lemmas and theorems are depicted in Figure~\ref{fig:dependence}. In the final part of the Appendix, Appendix~D, we present further simulation results.

\tikzstyle{block} = [rectangle, draw=black, fill=white, node distance=1.1cm, minimum height=2em, font=\color{black}\sffamily, rounded corners=5pt, text width=6em, text badly centered]
\tikzstyle{cloud} = [ellipse, draw=black, fill=white, node distance=1.1cm, minimum height=2em, font=\color{black}\sffamily,text width=5em, text badly centered]
% \tikzstyle{line} = [draw, -latex']
\tikzstyle{line} = [draw, -latex', line width=0.2mm, preaction={-triangle 90, thin, draw, shorten >=-0.1mm}]

\begin{figure}[h]
\centering
\begin{tikzpicture}[auto, node distance=1.5cm]
    \node [cloud] (A2) {Lemma~\ref{cones_cond}};
    \node [cloud, right = of A2] (A1) {Theorem~\ref{lemma:duality_gap}};
  %  \node [cloud, right = of A2] (A3) {Lemma~\ref{re:nonzero}};
%     \node [cloud, right = of A3] (A4) {Lemma~\ref{re:subgradientinequality}};
    \coordinate (Middle) at ($(A2)!0.5!(A1)$);
 %    \coordinate (Middlep) at ($(A3)!0.5!(A4)$);
     \node [cloud, below = of Middle] (A3) {Theorem~\ref{thm:sup_norm_vdiff_main}};
     \node [block, right = of A3] (Thm1) {Theorem~\ref{thm:optimality}};
    % \node [block, right = of Thm1] (Thm2) {Theorem~\ref{Thm:AV}};
    % \coordinate (Middle) at ($(A3)!0.8!(Thm1)$);
    %\node [block>, below = of Middlep] (Thm) {Theorem~\ref{r:finalbound}};
  %  \path [line] (A1) -- (A2);
%    \path [line] (A3) -- (Thm);
%    \path [line] (A4) -- (Thm);
    \path [line] (A2)  -- (A3);
    \path [line] (A1) -- (Thm1);
    \path [line] (A3) -- (Thm1);
    % \draw (Thm1) -- (Thm2);
\end{tikzpicture}
\caption{Dependencies among the lemmas and theorems. For example, the arrow between Lemma~\ref{cones_cond} and Theorem~\ref{thm:sup_norm_vdiff_main} indicates that Theorem~\ref{thm:sup_norm_vdiff_main} relies on Lemma~\ref{cones_cond}.}
\label{fig:dependence}
\end{figure}

\section*{Appendix A. Underlying statistical results}
In this section, we derive two properties of all vectors close to a lasso solution: 
In Lemma~\ref{cones_cond}, we show that their error belongs to a cone; in Theorem~\ref{thm:sup_norm_vdiff_main}, we show that they satisfy an oracle inequality in $\ell_\infty$-norm.    

\begin{lemma}\label{cones_cond}
Let $\dif\geq 0$ be a constant, $\tuningparameter\geq 2\tuningparameter_\alpha$ a tuning parameter, and $\cm\in\Rp$ any vector that satisfies $f(\cm,\tuningparameter)\leq f(\tm,\tuningparameter)+\dif$. Then $\vdiff:=\tm-\cm$ belongs to the cone
\begin{equation*}
    \cones:= \left\{\nu\in\R^p\,:\,\normone{\nu_{\setsc}}\leq \coneparam\normone{\nu_{\sets}} + \coneparamb \right\}\,.
\end{equation*}
\end{lemma}

\begin{proof}[Lemma~\ref{cones_cond}]
Since $f(\cm,\tuningparameter)\leq f(\tm,\tuningparameter)+\dif \leq f(\tmdt,\tuningparameter)+\dif$\,, we find the basic inequality
\begin{equation*}
  \normtwo{Y-X\cm}^2+\tuningparameter\normone{\cm}\leq \normtwo{Y-X\tmdt}^2+\tuningparameter\normone{\tmdt}+\dif\,.
\end{equation*}
We can now rewrite $\normtwo{Y-X\cm}^2$ as follows:
\begin{align*}
    \normtwo{Y-X\cm}^2 &= \normtwo{Y-X\tmdt+X\tmdt-X\cm}^2\\
    &= \normtwo{Y-X\tmdt}^2 + 2\inprod{Y-X\tmdt}{X\tmdt-X\cm}+ \normtwo{X\tmdt-X\cm}^2\\
    &= \normtwo{Y-X\tmdt}^2 + 2\inprod{X^\top(Y-X\tmdt)}{\tmdt-\cm}+ \normtwo{X\tmdt-X\cm}^2\,.
\end{align*}
Combining the two displays yields
\begin{align*}
2\inprod{X^\top(Y-X\tmdt)}{\tmdt-\cm}+    \normtwo{X\tmdt-X\cm}^2+\tuningparameter\normone{\cm} 
    &\leq \tuningparameter\normone{\tmdt}+\dif\,,
\end{align*}
and, by rearranging and using that $\normtwo{X\tmdt-X\cm}^2\geq 0$,
\begin{align*}
\tuningparameter\normone{\cm}
    &\leq \inprod{2X^\top(Y-X\tmdt)}{\cm-\tmdt} +    \tuningparameter\normone{\tmdt}+\dif\,.
\end{align*}
Invoking  H\"older's inequality and the KKT conditions for $\tmdt$ provides us with
\begin{align*}
  2\inprod{X^\top(Y-X\tmdt)}{\cm-\tmdt} &\leq \normsup{2X^\top(Y-X\tmdt)}\normone{\cm-\tmdt}\\
&\leq\frac{\tuningparameter}{2}\normone{\cm-\tmdt}\,.
\end{align*}
Combining the two displays yields
\begin{align*}
 2\normone{\cm} &\leq \normone{\cm-\tmdt}+2\normone{\tmdt}+\frac{2\dif}{\tuningparameter}\,.
\end{align*}
Hence,
\begin{align*}
    2\normone{\cmh}+2\normone{\cmhc} &\leq \normone{\cmh-\tmhdt}+\normone{\cmhc-\tmdthc}+2\normone{\tmhdt}+2\normone{\tmdthc}+\frac{2\dif}{\tuningparameter}\\ 
&=\normone{\cmh-\tmhdt}+\normone{\cmhc}+2\normone{\tmhdt}+\frac{2\dif}{\tuningparameter}\,,
\end{align*}
where $\seth:=\operatorname{supp}(\tmdt).$ This is equivalent to
\begin{align*}
    \normone{\cmhc} &\leq \normone{\cmh-\tmhdt}+2\normone{\tmhdt}-2\normone{\cmh}+\frac{2\dif}{\tuningparameter}\,,
\end{align*}
so that with the reverse triangle inequality
\begin{align*}
    \normone{\cmhc} &\leq 3\normone{\cmh-\tmhdt}+\frac{2\dif}{\tuningparameter}\,. 
\end{align*}
Finally, setting $\vdiff:=\tm-\cm,$ we get 
\begin{align*}
    \normone{\vdiffhc} &\leq 3\normone{\vdiffh}+\frac{2\dif}{\tuningparameter}\,. 
\end{align*}
Now, since $\tuningparameter/2\geq \tuningparameter_\alpha,\,$ Condition~1.1~(i)  entails $\normone{\vdiffh} \leq \normone{\vdiffs}$ and $\normone{\vdiffsc} \leq \normone{\vdiffhc}$. Combining these two inequalities with the above display yields
\begin{align*}
    \normone{\vdiffsc} &\leq \normone{\vdiffhc} \leq \coneparam\normone{\vdiffh} + \coneparamb \leq \coneparam\normone{\vdiffs} + \coneparamb
\end{align*}
as desired.
\end{proof}
\begin{theorem}\label{thm:sup_norm_vdiff_main}
Suppose that $\alpha>0$ and $\tuningparameter\geq 2\tuningparameter_\alpha$. Then, for any $\dif\geq 0$ and any $\cm\in\Rp$ with $f(\cm,\tuningparameter)\leq f(\tm,\tuningparameter)+\dif,$ it holds with probability at least $1-\alpha$ that  
\begin{equation*}
 \normsup{\truth-\cm}\leq \frac{\supc\tuningparameter}{ \nobs}+\sqrt{\frac{\dif}{\nobs\re}}\,.
\end{equation*}
\end{theorem}
\begin{proof}[Theorem~\ref{thm:sup_norm_vdiff_main}]
In view of Condition~1.1~(ii), it is sufficient to show that 
\begin{equation*}
 \normsup{\tm-\cm}\leq \sqrt{\frac{\dif}{\nobs\re}}\,.
\end{equation*}
Indeed, the desired claim follows directly from this via the triangle inequality for norms.

Let us prove the above inequality. Since $f(\tm,\tuningparameter)\leq f(\cm,\tuningparameter)\leq f(\tm,\tuningparameter)+\dif,\,$ we find the basic equality
\begin{align*}
 \normtwo{Y-X\cm}^2+\tuningparameter\normone{\cm}=   \normtwo{Y-X\tm}^2+\tuningparameter\normone{\tm}+\dift\,,
\end{align*}
for some $\dift\in[0,\dif].$ This equation is equivalent to
\begin{align*}
 \normtwo{Y-X\tm+X\tm-X\cm}^2+\tuningparameter\normone{\cm}=  \normtwo{Y-X\tm}^2 +\tuningparameter\normone{\tm}+\dift\,,
\end{align*}
and hence to
\begin{align*}
 \normtwo{Y-X\tm}^2+ 2\inprod{Y-X\tm}{X\tm-X\cm}+ \normtwo{X\tm-X\cm}^2+\tuningparameter\normone{\cm}=  \normtwo{Y-X\tm}^2 +\tuningparameter\normone{\tm}+\dift\,,
\end{align*}
and finally
\begin{align*}
 \normtwo{Y-X\tm}^2+ \inprod{2X^\top(Y-X\tm)}{\tm-\cm}+ \normtwo{X\tm-X\cm}^2+\tuningparameter\normone{\cm}=  \normtwo{Y-X\tm}^2 +\tuningparameter\normone{\tm}+\dift\,.
\end{align*}
Rearranging yields
\begin{align*}
\normtwo{X\tm-X\cm}^2=\inprod{2X^\top(Y-X\tm)}{\cm-\tm}-\tuningparameter\normone{\cm}+\tuningparameter\normone{\tm}+\dift\,.
\end{align*}
We now recall that the KKT conditions for the objective function $f$ read
\begin{equation*}
  -2X^\top(Y-X\tm)+\tuningparameter\vsub=0
\end{equation*} 
for any vector $\vsub$ that satisfies $\normsup{\vsub}\leq 1$ and $\vsub^\top\tm = \normone{\tm}$. %$\vsub_j=\sign(\tm_j)$ if $\tm_j\neq 0.$ 
Plugging this into the above display yields
\begin{align*}
\normtwo{X\tm-X\cm}^2 &= \inprod{\tuningparameter\vsub}{\cm-\tm}-\tuningparameter\normone{\cm}+\tuningparameter\normone{\tm}+\dift\\
&= \tuningparameter(\vsub^\top\cm - \normone{\cm})+\dift\,,
\end{align*}
and by H\"older's inequality, $\vsub^\top\cm\leq \normsup{\vsub}\normone{\cm} \leq \normone{\cm}$\,.

Therefore,
\begin{align*}
\normtwo{X\tm-X\cm}^2\leq \dift\leq \dif\,.
\end{align*}
We finally get, setting $\vdiff:=\tm-\cm,$
\begin{align*}
\normtwo{X\vdiff}^2 &\leq \dif\,.
\end{align*}
Moreover, Lemma~\ref{cones_cond} guarantees that $\vdiff\in\cones$ and thus allows us to apply Condition~2.1. So we also find 
\begin{equation*}
    \normtwo{X\vdiff}^2 \geq \nobs\re\normtwo{\vdiff}^2\,.
\end{equation*}
Combining these two inequalities gives us
\begin{equation*}
    \normtwo{\vdiff}^2 \leq \frac{\dif}{\nobs\re}\,,
\end{equation*}
which implies 
\begin{equation*}
    \normsup{\vdiff}\leq \sqrt{\frac{\dif}{\nobs\re}}
\end{equation*}
as desired.
\end{proof}

==> sections/suppl_exp.tex <==
\section*{Appendix D. Additional simulation results}

We provide additional simulation results to complement the empirical studies in the main part of the paper. We consider the $n=500$ and $p=1000$ setting with the specifications as described in the main part of the paper - except for the stated differences.

In Table~\ref{tabadd}, we add the results for Lasso with AIC and BIC. In Table~\ref{tabS}, we consider different support sizes. In Table~\ref{tabr}, we vary the correlation. 



The BIC and AIC criteria are defined as in~\cite{Zou07}:
\begin{align*}
    \text{BIC}(\tuningparameter) &= \frac{\normtwo{Y-X\cm^{\tuningparameter}}^2}{\nobs\sigma^2_\varepsilon}+\frac{\log(\nobs)|\settilde^{\tuningparameter}|}{\nobs}\\
    \text{AIC}(\tuningparameter) &= \frac{\normtwo{Y-X\cm^{\tuningparameter}}^2}{\nobs\sigma^2_\varepsilon}+\frac{2|\settilde^{\tuningparameter}|}{\nobs}\,,
\end{align*}
where $\sigma^2_\varepsilon$ is the variance of the noise $\varepsilon$. In our experiments, $\sigma^2_\varepsilon=1$. To establish valid comparisons, we again implement these schemes with the \texttt{SPAMS} package.

\begin{table}%[!ht]
  \centering
  %\vspace{.5\baselineskip}
%   \fbox{
  \begin{tabular}{lll}
    \toprule
    % & \multicolumn{2}{c}{$|\sets|=5$} & \multicolumn{2}{c}{$|\sets|=30$}                  \\
    % \cmidrule{2-3}
    Method     & Timing     & Hamming distance \\
    % \midrule
    \hline
    \lcvs & $137.15\pm 9.33$  &  $56.00\pm 18.37$  \\
    \lcvg     & $~~~2.08\pm 0.32$ & $44.90\pm 16.07$ \\
    \lbics     & $~\,20.12\pm 5.98$ & $10.40\pm ~\,7.15$  \\
    \laics     & $~\,20.12\pm 5.98$ & $45.30\pm21.40$\\
    FOS     & $~~\,\,0.10\pm 0.06$       & $~\,8.60\pm~\,3.10$\\
    \bottomrule
  \end{tabular}
%   }
\caption{\label{tabadd}Average run times (in seconds) and average Hamming distances for \lcvs, \lcvg, \lbics, \laics, and FOS.}
\end{table}

\begin{table}%[!ht]
\centering
%  \vspace{.5\baselineskip}
% \fbox{
  \begin{tabular}{lllll}
    \toprule
    & \multicolumn{2}{c}{$|\sets|=5$} & \multicolumn{2}{c}{$|\sets|=30$}                  \\
%    \cmidrule{2-5}
	\cline{2-5}
    Method     & Timing     & Hamming distance & Timing     & Hamming distance\\
%    \midrule
	\hline
    \lcvs & $283.19\pm 75.41$  &  $43.50\pm 19.53$  & $224.92\pm 41.77$  &$117.50\pm 22.49$\\
    \lcvg     & $~~~2.59\pm~\,0.40$ & $29.90\pm 12.66$    & $~~~2.52\pm~~0.25$ & $~\,98.00\pm 35.50$  \\
    FOS     & $~~~0.76\pm~\,2.13$       & $~\,4.40\pm~\,1.58$ & $~~~2.23\pm~~2.01$      & $~\,20.60\pm 11.98$ \\
    \bottomrule
  \end{tabular}
%   }
  \caption{Average run times (in seconds) and average Hamming distances for \lcvs, \lcvg, and FOS for two different sizes of the true support: $|\sets|\in\{5,30\}$. \label{tabS}}
\end{table}

\begin{table}%[!ht]
  \centering
%  \vspace{.5\baselineskip}
% \fbox{
  \begin{tabular}{lllll}
    \toprule
    & \multicolumn{2}{c}{$\rho=0$} & \multicolumn{2}{c}{$\rho=0.4$}                  \\
%    \cmidrule{2-5}
	\cline{2-5}
    Method     & Timing     & Hamming distance & Timing     & Hamming distance\\
%    \midrule
	\hline
    \lcvs & $168.03\pm 25.28$  &  $56.50\pm 22.45$  & $177.79\pm 48.11$  & $58.30\pm 20.67$\\
    \lcvg     & $~~~2.46\pm~\,0.24$ & $40.40\pm 13.17$    & $~~~2.36\pm~\,0.21$ & $44.50\pm 18.12$  \\
    FOS     & $~~~1.78\pm~\,0.73$       & $~\,1.10\pm~\,1.29$ & $~~~0.12\pm~\,0.06$      & $~\,9.70\pm~\,0.95$ \\
    \bottomrule
  \end{tabular}
%  } 
\caption{Average run times (in seconds) and average Hamming distances for \lcvs, \lcvg, and FOS for two different strengths of the pairwise correlations: $\rho\in\{0,0.4\}$. \label{tabr}}
  \end{table}




==> sections/theory.tex <==
% \clearpage

\section{Statistical guarantees}\label{theory}
Variable selection is a common statistical technique; yet, standard approaches based on the lasso, SCAD, or MCP  lack finite sample guarantees. The reason is that these approaches involve one or more tuning parameters, and corresponding calibration schemes such as Cross-Validation are not equipped with corresponding theory. Similarly,  bounds for feature selection with methods such as the Square-Root lasso, see~\citet{Yoyo13}, presume knowledge of inaccessible model parameters such as the noise distribution. 

In strong contrast, our main result states that FOS is, up to small constant, equipped with the same statistical guarantees as the lasso with optimal, in practice unknown tuning parameter. Indeed, we have the following.
\begin{theorem}[Optimality of FOS]\label{thm:optimality} Consider $\cm^{\widetilde\tuningparameter}$ and \settilde\ returned by Algorithm~\ref{algo}. For any $\alpha>0,$ it holds with probability at least $1-\alpha$ that 
\begin{equation*}
      \normsup{\truth-\tilde\beta^{\tilde r}}\leq \frac{6(\supc+\supcomp/\sqrt{\re})\tuningparameter_\alpha}{ \nobs}\,.
\end{equation*}
Moreover, it holds with probability at least $1-\alpha$ that $\tilde r\leq 2r_\alpha$ and, if $\min_{j\in\sets}|\truth_j|>6(\supc+\supcomp/\sqrt{\re})\tuningparameter_{\alpha}/\nobs,$ that
\begin{equation*}
 \settilde\supset \sets\,.
\end{equation*}
\end{theorem}
\noindent This result proves three features of FOS: (1)~Entry-wise control: the coefficient estimates associated with FOS are accurate; in particular, any coefficients corresponding to false positives are small. (2)~False positive control: if FOS has false positives, the corresponding parameter values are bounded by ${6(\supc+\supcomp/\sqrt{\re})\tuningparameter_\alpha}/{ \nobs},$ that is, are very small. (3)~False negative control: FOS recovers all sufficiently large coefficients.  

Note that the result holds for any $\alpha>0,$ while $\alpha$ does {\it not} need to be specified in FOS. Note also that, opposed to the Square-Root lasso/Scaled lasso approach, the noise distribution does {\it not} need to be known beforehand.

Instead, the parameters that go into the algorithm are \supc, \re, and \supcomp. The values for \supc\ and \re\ are dictated by the theory. Indeed, it is well known that the lasso verifies Condition~\ref{boundcon} with $\supc=0.75$ for orthogonal design, and more generally, with $\supc\approx 0.75$ if the correlations are not too large~\citep{Karim08}. Similarly, Condition~\ref{RE} is verified with $\re=1$ for orthogonal design, and more generally, with $\re\approx 1$ if the correlations are not too large~\citep{vandeGeer14}. Since $\ell_\infty$-estimation and support recovery are not possible altogether if the correlations are large~\citep{BiYuConsistlasso}, we can thus set $\supc=0.75$ and $\re=1$ for all practical purposes. The value for \supcomp\ is now found by balancing the statistical and computational precision. Indeed, the bounds are sharp as long as $\supcomp$ is at most of the order of $\supc.$ Thus, with the additional goal of computational efficiency in mind, the optimal value is $\supcomp\approx\supc,$ and we thus set $\supcomp=\supc$ for all practical purposes. In summary, we keep the constants \supc, \re, and \supcomp\ to highlight their role in the theory; however, they are not tuning parameters but instead dimensionless constants with values specified by theory.

The optimality of the scheme can be seen when comparing the $\ell_\infty$-bound with the corresponding bound in Condition~\ref{boundcon}. Indeed, our scheme satisfies the same bound as the lasso with optimal tuning parameter -  up to a small constant factor and without any additional log-terms or such\footnote{The constant can  be reduced even further by invoking a stronger cone condition; we omit the details to avoid digression.}.

We defer the proof of Theorem~\ref{thm:optimality} to the Appendix. It consists of three parts: First, we derive an oracle inequality for vectors that are  close to a lasso solution. Second, we use Fenchel duality~\citep{Borwein2010,Rifkin2007} to show that our scheme is sufficiently accurate. Finally, we show that the tuning parameters are calibrated optimally.
